A DESGW Search for the Electromagnetic Counterpart to the LIGO/Virgo Gravitational Wave Binary Neutron Star Merger Candidate S190510g

We present the results from a search for the electromagnetic counterpart of the LIGO/Virgo event S190510g using the Dark Energy Camera (DECam). S190510g is a binary neutron star (BNS) merger candidate of moderate significance detected at a distance of 227$\pm$92 Mpc and localized within an area of 31 (1166) square degrees at 50\% (90\%) confidence. While this event was later classified as likely non-astrophysical in nature within 30 hours of the event, our short latency search and discovery pipeline identified 11 counterpart candidates, all of which appear consistent with supernovae following offline analysis and spectroscopy by other instruments. Later reprocessing of the images enabled the recovery of 6 more candidates. Additionally, we implement our candidate selection procedure on simulated kilonovae and supernovae under DECam observing conditions (e.g., seeing, exposure time) with the intent of quantifying our search efficiency and making informed decisions on observing strategy for future similar events. This is the first BNS counterpart search to employ a comprehensive simulation-based efficiency study. We find that using the current follow-up strategy, there would need to be 19 events similar to S190510g for us to have a 99\% chance of detecting an optical counterpart, assuming a GW170817-like kilonova. We further conclude that optimization of observing plans, which should include preference for deeper images over multiple color information, could result in up to a factor of 1.5 reduction in the total number of followups needed for discovery.

==> KNpaperCommands.tex <==
\newcommand{\snana}{{{\tt SNANA}}}
\newcommand{\simlib}{{\tt SIMLIB}}
\newcommand{\as}{{\tt autoScan}}
\newcommand{\ler}{$4\times 10^{-3}$} % probability of finding KN assuming 2 seasons
\newcommand{\her}{1-2} % detections per year assuming high rate
\newcommand{\ligorate}{$1.26\times10^{4}$ yr$^{-1}$Gpc$^{-3}$}
\newcommand{\grbrate}{$10$ yr$^{-1}$Gpc$^{-3}$}
\newcommand{\grbrateFong}{$90$ yr$^{-1}$Gpc$^{-3}$}
\newcommand{\grbrateFongFull}{$270^{+1580}_{-180}$ yr$^{-1}$Gpc$^{-3}$}
\newcommand{\diffimg}{{\tt DiffImg}}
\newcommand{\zphot}{$z_{\rm phot}$}
\newcommand{\diz}{$\delta_{iz}$}
\newcommand{\shallowTrigs}{3487} % number of KN triggers in shallow
\newcommand{\deepTrigs}{1236} % number of KN triggers in deep fields
\newcommand{\maxKNratelim}{1.0$\times 10^{7}$ Gpc$^{-3}$yr$^{-1}$} % the higher upper rate limit we set
\newcommand{\minKNratelim}{2.4$\times 10^{4}$ Gpc$^{-3}$yr$^{-1}$} % the lower upper rate limit we set
\newcommand{\maxKNratelimd}{4.6$\times 10^{7} $ Gpc$^{-3}$yr$^{-1}$} % the higher upper rate limit we set
\newcommand{\minKNratelimd}{5.2$\times 10^{4} $Gpc$^{-3}$yr$^{-1}$} % the lower upper rate limit we set
\newcommand{\NCUTSDATA}{0}   % Number of data events passing all cuts
\newcommand{\NCUTSSIM}{$1.1\pm0.2$}  % number of SN sim events passing all cuts for SN simulation
\newcommand{\NPASSSND}{0.96}
\newcommand{\NPASSSNS}{0.17}
\newcommand{\NGENIa}{$3.7 \times 10^5$}
\newcommand{\NGENCC}{$4.3 \times 10^6$}
\newcommand{\mSB}{m_{\rm SB}}
\newcommand{\effKN}{\epsilon_{\rm KN}}
\newcommand{\NKN}{N_{\rm KN}}
\newcommand{\ZPmedian}{$\rm ZP_{median}$}
\newcommand{\shallowEcliptic}{42}
\newcommand{\shallowNoEcliptic}{11}
\newcommand{\deepEcliptic}{4}
\newcommand{\deepNoEcliptic}{4}
\newcommand{\SNSIMSCALE}{40}
\newcommand{\IaRedshift}{1.1}
\newcommand{\CCRedshift}{0.8}
\newcommand{\passColor}{0.66}
\newcommand{\dimmestpeakmagi}{$M_i = -11.4$}
\newcommand{\brightestpeakmagi}{$M_i = -16.2$}
\newcommand{\effdiffimg}{\epsilon_{\diffimg}}
\newcommand{\effsnana}{\epsilon_{\snana}}
\newcommand{\effnohost}{\epsilon_{{\rm No Host},\snana}}
\newcommand{\effnohostd}{\epsilon_{{\rm No Host},\diffimg}}
\newcommand{\effratio}{\mathcal{R}_\epsilon}
\newcommand{\KN}{{\small KN}}
\newcommand{\KNe}{{\small KN}e}
\newcommand{\LIGO}{{\small LIGO}}
\newcommand{\BK}{{\small BK}13}
\newcommand{\GW}{{\small GW}}
\newcommand{\EM}{{\small EM}}
\newcommand{\SN}{{\small SN}}
\newcommand{\SNe}{{\small SN}e}
\newcommand{\GRB}{{\small GRB}}
\newcommand{\SGRB}{{\small SGRB}}
\newcommand{\DESSN}{{\small DES}-{\small SN}}
\newcommand{\DES}{{\small DES}}
\newcommand{\BNS}{{\small BNS}}

